A Strong Distillery

Abstract machines for the strong evaluation of lambda-terms (that is, under abstractions) are a mostly neglected topic, despite their use in the implementation of proof assistants and higher-order logic programming languages. This paper introduces a machine for the simplest form of strong evaluation, leftmost-outermost (call-by-name) evaluation to normal form, proving it correct, complete, and bounding its overhead. Such a machine, deemed Strong Milner Abstract Machine, is a variant of the KAM computing normal forms and using just one global environment. Its properties are studied via a special form of decoding, called a distillation, into the Linear Substitution Calculus, neatly reformulating the machine as a standard micro-step strategy for explicit substitutions, namely linear leftmost-outermost reduction, i.e., the extension to normal form of linear head reduction. Additionally, the overhead of the machine is shown to be linear both in the number of steps and in the size of the initial term, validating its design. The study highlights two distinguished features of strong machines, namely backtracking phases and their interactions with abstractions and environments.

==> compat_abstraction_proof.tex <==
% !TEX root = main.tex
By induction on the derivation of $\var\cons\skframe \compatible \genv$.
There are three cases:
\begin{enumerate}
\item \casealt{Case $\genv = \esub{\var}{\skboundvar}\cons\genvthree$ with $\skframe \compatible \genvthree$}\\
      By taking $\genvtwo \defeq \stempty$ we have that $\genv = \genvtwo\cons\esub{\var}{\skboundvar}\cons\genvthree$.
      Moreover:
      $$
        \decodecompat{\var\cons\skframe}{\genv} = 
        \decodecompat{\var\cons\skframe}{\esub{\var}{\skboundvar}\cons\genvthree} = 
        \decodecompat{\skframe}{\genvthree}\ctxholep{\l\var.\ctxhole}
      $$
      as wanted.
\item \casealt{Case $\genv = \esub{\vartwo}{\code}\cons\genv_1$ with $\var \neq \vartwo$ and $\var\cons\skframe \compatible \genv_1$}\\
      By \ih, $\genv_1$ can be written as of the form $\genv_1 = \genvtwo_1\cons\esub{\var}{\skboundvar}\cons\genvthree$,
      where $\genvtwo_1$ is a \substitutive environment, $\skframe \compatible \genvthree$
      and $\decodecompat{\var\cons\skframe}{\genv_1} = \decodecompat{\skframe}{\genvthree}\ctxholep{\l\var.\decode{\genvtwo_1}}$.

      By taking $\genvtwo \defeq \esub{\vartwo}{\code}\cons\genvtwo_1$ we have that
      in fact $\genv = \genvtwo\cons\esub{\var}{\skboundvar}\cons\genvthree$,
      where $\esub{\vartwo}{\code}\cons\genvtwo_1$ is a \substitutive environment.
      The condition $\skframe \compatible \genvthree$ is already known to hold.
      Moreover:
      $$
        \begin{array}{rll}
            & \decodecompat{\skl\cons\skframe}{\genv} \\
          = & \decodecompat{\skl\cons\skframe}{\esub{\vartwo}{\code}\cons\genv_1} \\
          = & \decodecompat{\skl\cons\skframe}{\genv_1}\ctxholep{\ctxhole\esub{\vartwo}{\code}} \\
          = & \decodecompat{\skframe}{\genvthree}\ctxholep{\l\var.\decode{\genvtwo_1}\ctxholep{\ctxhole\esub{\vartwo}{\code}}} & \text{by \ih} \\
          = & \decodecompat{\skframe}{\genvthree}\ctxholep{\l\var.\decode{\esub{\vartwo}{\code}\cons\genvtwo_1}} \\
          = & \decodecompat{\skframe}{\genvthree}\ctxholep{\l\var.\decode{\genvtwo}} \\
        \end{array}
      $$
      as wanted.
\item \casealt{Case $\genv = \esub{\vartwo}{\skerased}\cons\genv_1\cons\esub{\vartwo}{\skboundvar}\cons\genv_2$ with $\var \neq \vartwo$ and $\var\cons\skframe \compatible \genv_2$}\\
      By \ih, $\genv_2$ can be written as of te form $\genv_2 = \genvtwo_2\cons\esub{\var}{\skboundvar}\cons\genvthree$,
      where $\genv_2$ is a substitutive environment, $\skframe \compatible \genvthree$ and
      $\decodecompat{\var\cons\skframe}{\genv_2} = \decodecompat{\skframe}{\genvthree}\ctxholep{\l\var.\decode{\genvtwo_2}}$

      By taking $\genvtwo \defeq \esub{\vartwo}{\skerased}\cons\genv_1\cons\esub{\vartwo}{\skboundvar}\cons\genvtwo_2$
      we have that in fact $\genv = \genvtwo\cons\esub{\var}{\skboundvar}\cons\genvthree$,
      where $\esub{\vartwo}{\skerased}\cons\genv_1\cons\esub{\vartwo}{\skboundvar}\cons\genvtwo_2$ is a \substitutive
      environment.
      The condition $\skframe \compatible \genvthree$ is already known to hold. Moreover:
      $$
        \begin{array}{rll}
            & \decodecompat{\skl\cons\skframe}{\genv} \\
          = & \decodecompat{\skl\cons\skframe}{\esub{\vartwo}{\skerased}\cons\genv_1\cons\esub{\vartwo}{\skboundvar}\cons\genvtwo_2\cons\esub{\var}{\skboundvar}\cons\genvthree} \\
          = & \decodecompat{\skl\cons\skframe}{\genvtwo_2\cons\esub{\var}{\skboundvar}\cons\genvthree} \\
          = & \decodecompat{\skframe}{\genvthree}\ctxholep{\l\var.\decode{\genvtwo_2}} \\
          = & \decodecompat{\skframe}{\genvthree}\ctxholep{\l\var.\decode{\esub{\vartwo}{\skerased}\cons\genv_1\cons\esub{\vartwo}{\skboundvar}\cons\genvtwo_2}} \\
          = & \decodecompat{\skframe}{\genvthree}\ctxholep{\l\var.\decode{\genvtwo}}
        \end{array}
      $$\qed
\end{enumerate}


==> compat_binding_proof.tex <==
% !TEX root = main.tex
\ben{to revisit, probably the induction can be simply on $\skframe$}.
By induction on the derivation of $\skframe \compatible \genv$.
The interesting case is when $\skframe = \skap{\codetwo}{\stack}\cons\skframetwo$ and
there is a derivation of $\skap{\codetwo}{\stack}\cons\skframetwo \compatible \genv$
whose premise is a derivation of $\skframetwo \compatible \genv$.

Then $\skap{\codetwo}{\stack}\cons\skframetwo \compatible \esub{\var}{\code}\cons\genv$ can be
derived from $\skframetwo \compatible \esub{\var}{\code}\cons\genv$ which is by
\ih\ a consequence of $\skframetwo \compatible \genv$.
Moreover, let $\skframetwo_{\mathrm h}$ and $\skframetwo_{\mathrm t}$ be the \structural and \tail of $\skframetwo$, respectively. Then:
$$
\begin{array}{rcl}
	\decodecompat{\skap{\codetwo}{\stack}\cons\skframetwo}{\esub{\var}{\code}\cons\genv} &=& 
	\decodecompat{\skframetwo}{\esub{\var}{\code}\cons\genv}\ctxholep{\decode{\skap{\codetwo}{\stack}}} =
	\decodecompat{\skframetwo_{\mathrm t}}{\genv}\ctxholep{\decode{\skframetwo_{\mathrm h}}\ctxholep{\decode{\skap{\codetwo}{\stack}}}\esub{\var}{\code}} \\
	& \stackrel{\textrm{\footnotesize by \ih}}{=} &
	\decodecompat{\skframetwo_{\mathrm t}}{\genv}\ctxholep{\decode{\skap{\codetwo}{\stack}\cons\skframetwo_{\mathrm h}}\esub{\var}{\code}}
\end{array}
$$
$$
  \begin{array}{rll}
      & \decodecompat{\skap{\codetwo}{\stack}\cons\skframetwo}{\esub{\var}{\code}\cons\genv} \\
    = & \decodecompat{\skframetwo}{\esub{\var}{\code}\cons\genv}\ctxholep{\decode{\skap{\codetwo}{\stack}}} \\
    = & \decodecompat{\skframetwo_{\mathrm t}}{\genv}\ctxholep{\decode{\skframetwo_{\mathrm h}}\ctxholep{\decode{\skap{\codetwo}{\stack}}}\esub{\var}{\code}}
      & \text{by \ih} \\
    = & \decodecompat{\skframetwo_{\mathrm t}}{\genv}\ctxholep{\decode{\skap{\codetwo}{\stack}\cons\skframetwo_{\mathrm h}}\esub{\var}{\code}}
  \end{array}
$$
We conclude by noting that $\skap{\codetwo}{\stack}\cons\skframetwo_{\mathrm h}$ and $\skframetwo_{\mathrm t}$ are the \structural and \tail of $\skframe$, respectively.\qed



==> proofs/close-name-invariant-proof.tex <==
% !TEX root = ../main.tex
\begin{proof}
  The invariant trivially holds for an initial state
  $\skamstate{\skeval}{\stempty}{\code_0}{\stempty}{\stempty}$, as $\code_0$ is assumed to be closed and well-named.
  For the inductive cases we consider the last transition $\state\tomach\statetwo$. We omit the cases for $\tomachcp{_{1,2,3,5,6}}$, because for them $\decode\state = \decode\statetwo$ holds, and so the statement follows from the \ih.
  \begin{itemize}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skeval}{\skframe}{\l\var.\code}{\codetwo\cons\stack}{\genv}
          \tomachm
          \mac{\skeval}{\skframe}{\code}{\stack}{\esub{\var}{\codetwo}\cons\genv}
        $}
      Let $\skframe = \skframeweak\cons\skframetrunk$. By \ih, the following term:
      $$
        \begin{array}{rll}
             \decodecompat{\skframe}{\genv}\ctxholep{\dstackp{(\l\var.\code)\codetwo}} 
           = & \decodecompat{\skframetrunk}{\genv}\ctxholep{\decode{\skframeweak}\ctxholep{\dstackp{(\l\var.\code)\codetwo}}}
        \end{array}
      $$
      is closed and well-named. The term we are interested in is:
      $$
        \begin{array}{rll}
            \decodecompat{\skframe}{\esub{\var}{\codetwo}\cons\genv}\ctxholep{\dstackp{\code}} &
          = & \decodecompat{\skframetrunk}{\genv}\ctxholep{\decode{\skframeweak}\ctxholep{\dstackp{\code}}\esub{\var}{\codetwo}} \\
        \end{array}.
      $$
      It is closed because in $\decode{\skframeweak}\ctxholep{\decode{\stack}}$ there are no binders and $\var$ does not occur by hypothesis, so that no scope violation can occur. It is also easily seen to be well-named since the rule
      is linear, \ie\ no subexpressions are duplicated.



  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skeval}{\skframe}{\var}{\stack}{\genv}
          \tomache
          \mac{\skeval}{\skframe}{\rename{\code}}{\stack}{\genv}
        $}
By \ih, $\decodecompat{\skframe}{\genv}\ctxholep{\dstackp{\var}}$ is closed and well-named.
      Then $\decodecompat{\skframe}{\genv}\ctxholep{\dstackp{\rename{\code}}}$ is also closed (because $\decodecompat{\skframe}{\genv}$ captures all the free variables of $\rename{\code}$) and well-named (since all the bound variables of $\rename{\code}$ are fresh).

    %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skback}{\var\cons\skframe}{\code}{\stempty}{\genv}
          \tomachasubfour
          \mac{\skback}{\skframe}{\l\var.\code}{\stempty}{\closescopem\var\cons\genv}
        $}
        
        From the proof of the distillation we have that $\decode\state = \decode{\mac{ \skback }{ \var\cons\skframe }{ \code }{ \stempty }{ \genv }}$ is equal to $\decode\statetwo = \decode{\mac{ \skback }{ \skframe }{ \l\var.\code }{ \stempty }{ \closescopem\var\cons\genv }}
$ up to some garbage collection. By \ih $\decode\state$ is closed and well named, and so $\decode\statetwo$ is closed and well named.\qed
  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

  \end{itemize}
\end{proof}

==> proofs/invariants-skeleton.tex <==
% !TEX root = ../main.tex
  The invariant trivially holds for an initial state
  $\skamstate{\skeval}{\stempty}{\code_0}{\stempty}{\stempty}$
  if $\code_0$ is closed and well-named.
For a non-empty evaluation sequence we list the cases for the last transitions:
  \begin{itemize}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skeval}{\skframe}{\code\codetwo}{\stack}{\genv}
          \tomachasubone
          \mac{\skeval}{\skframe}{\code}{\codetwo\cons\stack}{\genv}
        $}

%    \begin{enumerate}
%	\item
%    \end{enumerate}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skeval}{\skframe}{\l\var.\code}{\codetwo\cons\stack}{\genv}
          \tomachm
          \mac{\skeval}{\skframe}{\code}{\stack}{\esub{\var}{\codetwo}\cons\genv}
        $}
%    \begin{enumerate}
%	\item
%    \end{enumerate}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skeval}{\skframe}{\l\var.\code}{\stempty}{\genv}
          \tomachasubtwo
          \mac{\skeval}{\var\cons\skframe}{\code}{\stempty}{\openscopem\var\cons\genv}
        $}
%    \begin{enumerate}
%	\item
%    \end{enumerate}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skeval}{\skframe}{\var}{\stack}{\genv}
          \tomache
          \mac{\skeval}{\skframe}{\rename{\code}}{\stack}{\genv}
        $}
    
%    \begin{enumerate}
%	\item
%    \end{enumerate}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skeval}{\skframe}{\var}{\stack}{\genv}
          \tomachasubthree
          \mac{\skback}{\skframe}{\var}{\stack}{\genv}
        $}
    Note that $\genv(\var) = \skboundvar$, \ie\ $\var \in \skl(\genv)$.
%    \begin{enumerate}
%	\item
%    \end{enumerate}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skback}{\var\cons\skframe}{\code}{\stempty}{\genv}
          \tomachasubfour
          \mac{\skback}{\skframe}{\l\var.\code}{\stempty}{\closescopem\var\cons\genv}
        $}
        	By the compatibility invariant (\reflemmap{strong-mam-invariants}{comp}) $\var\cons\skframe \compatible \genv$, and by the factorization property of compatible pairs (\reflemmap{comp-properties}{fact}) $\genv = \genvweak\cons\openscopem\var\cons\genvtwo$. 
%    \begin{enumerate}
%	\item
%    \end{enumerate}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skback}{\skap{\code}{\stack}\cons\skframe}{\codetwo}{\stempty}{\genv}
          \tomachasubfive
          \mac{\skback}{\skframe}{\code\codetwo}{\stack}{\genv}
        $}
%    \begin{enumerate}
%	\item
%    \end{enumerate}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skback}{\skframe}{\code}{\codetwo\cons\stack}{\genv}
          \tomachasubsix
          \mac{\skeval}{\skap{\code}{\stack}\cons\skframe}{\codetwo}{\stempty}{\genv}
        $}
%    \begin{enumerate}
%	\item
%    \end{enumerate}

  \end{itemize}


==> proofs/well-formedness-invariant-proof.tex <==
% !TEX root = ../main.tex
  The invariant trivially holds for an initial state
  $\skamstate{\skeval}{\stempty}{\code_0}{\stempty}{\stempty}$
  if $\code_0$ is closed and well-named.
For a non-empty evaluation sequence we list the cases for the last transitions. The cases where the environment does not change are omitted, because they immediately follow from the \ih:
  \begin{itemize}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skeval}{\skframe}{\l\var.\code}{\codetwo\cons\stack}{\genv}
          \tomachm
          \mac{\skeval}{\skframe}{\code}{\stack}{\esub{\var}{\codetwo}\cons\genv}
        $}
        
%    \begin{enumerate}
%	\item



%    \end{enumerate}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skeval}{\skframe}{\l\var.\code}{\stempty}{\genv}
          \tomachasubtwo
          \mac{\skeval}{\var\cons\skframe}{\code}{\stempty}{\openscopem\var\cons\genv}
        $}
%    \begin{enumerate}
%	\item
%    \end{enumerate}


  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \item \case{$
          \mac{\skback}{\var\cons\skframe}{\code}{\stempty}{\genv}
          \tomachasubfour
          \mac{\skback}{\skframe}{\l\var.\code}{\stempty}{\closescopem\var\cons\genv}
        $}
        	By \reflemma{comp_invariant} $\var\cons\skframe \compatible \genv$, and by \refrem{comp-fact} $\genv = \genvweak\cons\openscopem\var\cons\genvtwo$. 
%    \begin{enumerate}
%	\item
%    \end{enumerate}

  %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
  \end{itemize}

